B-Splines for Sparse Grids: Algorithms and Application to Higher-Dimensional Optimization

In simulation technology, computationally expensive objective functions are often replaced by cheap surrogates, which can be obtained by interpolation. Full grid interpolation methods suffer from the so-called curse of dimensionality, rendering them infeasible if the parameter domain of the function is higher-dimensional (four or more parameters). Sparse grids constitute a discretization method that drastically eases the curse, while the approximation quality deteriorates only insignificantly. However, conventional basis functions such as piecewise linear functions are not smooth (continuously differentiable). Hence, these basis functions are unsuitable for applications in which gradients are required. One example for such an application is gradient-based optimization, in which the availability of gradients greatly improves the speed of convergence and the accuracy of the results. This thesis demonstrates that hierarchical B-splines on sparse grids are well-suited for obtaining smooth interpolants for higher dimensionalities. The thesis is organized in two main parts: In the first part, we derive new B-spline bases on sparse grids and study their implications on theory and algorithms. In the second part, we consider three real-world applications in optimization: topology optimization, biomechanical continuum-mechanics, and dynamic portfolio choice models in finance. The results reveal that the optimization problems of these applications can be solved accurately and efficiently with hierarchical B-splines on sparse grids.

==> tex/preamble/settings.tex <==
\makeatletter

\input{tex/preamble/settings/metaData}
\input{tex/preamble/settings/komaTextArea}
\input{tex/preamble/settings/graphics}
\input{tex/preamble/settings/crossReferences}
\input{tex/preamble/settings/toc}
\input{tex/preamble/settings/minitoc}
\input{tex/preamble/settings/headings}
\input{tex/preamble/settings/dictums}
\input{tex/preamble/settings/headerFooter}
\input{tex/preamble/settings/initials}
\input{tex/preamble/settings/floats}
\input{tex/preamble/settings/captions}
\input{tex/preamble/settings/tables}
\input{tex/preamble/settings/algorithms}
\input{tex/preamble/settings/theorems}
\input{tex/preamble/settings/mathematics}
\input{tex/preamble/settings/dummyText}
\input{tex/preamble/settings/dynamic}
\input{tex/preamble/settings/text}
\input{tex/preamble/settings/colors}
\input{tex/preamble/settings/checkMode}
\input{tex/preamble/settings/flipBook}
\input{tex/preamble/settings/watermarks}
\input{tex/preamble/settings/hyperref}
\input{tex/preamble/settings/bibliography}
\input{tex/preamble/settings/glossary}

\makeatother


==> tex/preamble/settings/algorithms.tex <==
% ======================================================================
% Algorithms
% ======================================================================

% disable ligatures ("fi" etc.) in monospace font
\DisableLigatures{encoding=*,family=tt*}

% line number format
\algrenewcommand{\alglinenumber}[1]{\footnotesize\color{anthrazit}{\texttt{#1}}}
\algrenewcommand{\algorithmicrequire}{\textbf{Input:}}
\algrenewcommand{\algorithmicensure}{\textbf{Output:}}

% function name
\algrenewcommand{\textproc}{}

% bold keywords
\algnewcommand{\Break}{\textbf{break}}
\algnewcommand{\Continue}{\textbf{continue}}
\algnewcommand{\True}{\textbf{true}}
\algnewcommand{\False}{\textbf{false}}
\algnewcommand{\Null}{\textbf{null}}
\algrenewcommand{\algorithmicend}{\textbf{end}}
\algrenewcommand{\algorithmicdo}{\textbf{do}}
\algrenewcommand{\algorithmicwhile}{\textbf{while}}
\algrenewcommand{\algorithmicfor}{\textbf{for}}
\algrenewcommand{\algorithmicforall}{\textbf{for all}}
\algrenewcommand{\algorithmicloop}{\textbf{loop}}
\algrenewcommand{\algorithmicrepeat}{\textbf{repeat}}
\algrenewcommand{\algorithmicuntil}{\textbf{until}}
\algrenewcommand{\algorithmicprocedure}{\textbf{procedure}}
\algrenewcommand{\algorithmicfunction}{\textbf{function}}
\algrenewcommand{\algorithmicif}{\textbf{if}}
\algrenewcommand{\algorithmicthen}{\textbf{then}}
\algrenewcommand{\algorithmicelse}{\textbf{else}}
\algrenewcommand{\algorithmicreturn}{\textbf{return}}
\algnewcommand{\algorithmicforever}{\textbf{for ever}}
\algdef{S}[FOR]{ForEver}{\algorithmicforever\ \algorithmicdo}
\algnewcommand{\algorithmicgoto}{\textbf{go to}}
\algnewcommand{\Goto}[1]{\algorithmicgoto\ \cref*{#1}}
\algnewcommand{\ForOneLine}[2]{%
  \State\algorithmicfor\ #1\ \algorithmicdo\ #2%
}
\algnewcommand{\IfOneLine}[2]{%
  \State\algorithmicif\ #1\ \algorithmicthen\ #2%
}
\algnewcommand{\ElseOneLine}[1]{%
  \State\algorithmicelse\ #1%
}

% small monospace font in algorithms
\g@addto@macro\ALG@beginalgorithmic{\small\ttfamily}

% comment format
\algrenewcomment[1]{\hfill$\rightsquigarrow$\;{\normalfont\emph{#1}}}

% set indentation to two characters
\algrenewcommand{\algorithmicindent}{\widthof{AB}}

% make ALG@line.XX counters unique,
% otherwise hyperlinks to algorithm lines won't work
% (they will always point to the line with the same number,
% but in the first algorithm of the thesis)
\newcounter{algorithmicH}
\let\oldalgorithmic\algorithmic
\renewcommand*{\algorithmic}{\stepcounter{algorithmicH}\oldalgorithmic}
\renewcommand*{\theHALG@line}{ALG@line.\thealgorithmicH.\arabic{ALG@line}}


==> tex/preamble/settings/bibliography.tex <==
% ======================================================================
% Bibliography
% ======================================================================

% location of *.bib file
\addbibresource{bibliography.bib}

% include brackets in \cite hyperlink
\DeclareCiteCommand{\cite}{\usebibmacro{prenote}}{%
  \usebibmacro{citeindex}%
  \printtext[bibhyperref]{\mkbibbrackets{\usebibmacro{cite}}}%
}{\multicitedelim}{\usebibmacro{postnote}}

% declare special \multicite command which produces [Abc01; Def02]
% (instead of [Abc01]; [Def02])
\DeclareCiteCommand{\multicite}[\mkbibbrackets]{\usebibmacro{prenote}}{%
  \usebibmacro{citeindex}\usebibmacro{cite}%
}{\multicitedelim}{\usebibmacro{postnote}}

% don't append "+" sign to BibLaTeX citations in alphabetic style
\renewcommand*{\labelalphaothers}{}

% define custom heading to add bibliography to table of contents
\defbibheading{myheading}[\bibname]{\addchap{#1}}

% add custom bibliography post note (reset font size)
\defbibnote{mypostnote}{%
  \renewcommand*{\texttt}[1]{\oldtexttt{##1}}%
}

% order entries by last names
\DeclareNameAlias{sortname}{last-first}
\DeclareNameAlias{default}{last-first}

% change font size of bibliography
\renewcommand*{\bibfont}{\small}

% set single line spacing for bibliography
\renewcommand*{\bibsetup}{\singlespacing}

% separate authors with semicolon, suppress "and" in author names
\renewcommand*{\multinamedelim}{\addsemicolon\space}
\renewcommand*{\finalnamedelim}{\addsemicolon\space}

% make names bold
\renewcommand*{\mkbibnamefamily}[1]{\textbf{#1}}

% insert colon after author names in bibliography
\renewcommand*{\labelnamepunct}{\addcolon\space}

% separate BibLaTeX units with commas instead of periods
\renewcommand*{\newunitpunct}{\addcomma\space}

% make paper titles italic, remove quotation marks
\DeclareFieldFormat[article]{title}{\mkbibemph{#1}}
\DeclareFieldFormat[article]{journaltitle}{#1}
\DeclareFieldFormat[article]{issuetitle}{#1}
\DeclareFieldFormat[article]{issuesubtitle}{#1}
\DeclareFieldFormat[inbook]{title}{\mkbibemph{#1}}
\DeclareFieldFormat[inbook]{booktitle}{#1}
\DeclareFieldFormat[inbook]{maintitle}{#1}
\DeclareFieldFormat[incollection]{title}{\mkbibemph{#1}}
\DeclareFieldFormat[incollection]{booktitle}{#1}
\DeclareFieldFormat[incollection]{maintitle}{#1}
\DeclareFieldFormat[inproceedings]{title}{\mkbibemph{#1}}
\DeclareFieldFormat[inproceedings]{booktitle}{#1}
\DeclareFieldFormat[inproceedings]{maintitle}{#1}
\DeclareFieldFormat[inreference]{booktitle}{#1}
\DeclareFieldFormat[inreference]{maintitle}{#1}
\DeclareFieldFormat[thesis]{title}{\mkbibemph{#1}}
\DeclareFieldFormat[unpublished]{title}{\mkbibemph{#1}}

% fix title capitalization to sentence case (all lowercase)
\DeclareFieldFormat{titlecase}{\MakeTitleCase{#1}}

% .. but don't change journal titles, book titles, and so on
\newrobustcmd{\MakeTitleCase}[1]{%
  \ifthenelse{%
    \ifcurrentfield{booktitle}\OR\ifcurrentfield{booksubtitle}%
    \OR\ifcurrentfield{maintitle}\OR\ifcurrentfield{mainsubtitle}%
    \OR\ifcurrentfield{journaltitle}\OR\ifcurrentfield{journalsubtitle}%
    \OR\ifcurrentfield{issuetitle}\OR\ifcurrentfield{issuesubtitle}%
    \OR\ifentrytype{book}\OR\ifentrytype{mvbook}\OR\ifentrytype{bookinbook}%
    \OR\ifentrytype{booklet}\OR\ifentrytype{suppbook}%
    \OR\ifentrytype{collection}\OR\ifentrytype{mvcollection}%
    \OR\ifentrytype{suppcollection}\OR\ifentrytype{manual}%
    \OR\ifentrytype{periodical}\OR\ifentrytype{suppperiodical}%
    \OR\ifentrytype{proceedings}\OR\ifentrytype{mvproceedings}%
    \OR\ifentrytype{reference}\OR\ifentrytype{mvreference}%
    \OR\ifentrytype{thesis}\OR\ifentrytype{online}%
  }{%
    #1%
  }{%
    \MakeSentenceCase*{#1}%
  }%
}

% suppress "In:" before journal names
\renewbibmacro*{in:}{}

% don't put parentheses around year for journals
\renewbibmacro*{issue+date}{%
  \setunit{\addcomma\space}%
  \iffieldundef{issue}{%
    \usebibmacro{date}%
  }{%
    \printfield{issue}\setunit*{\addspace}\usebibmacro{date}%
  }%
  \newunit%
}

% reformat and link URLs, DOIs, and ISBNs
\DeclareFieldFormat{url}{\scriptsize\url{#1}}
\DeclareFieldFormat{doi}{%
  \scriptsize%
  \ifhyperref{%
    \href{https://doi.org/#1}{\nolinkurl{doi:#1}}%
  }{\nolinkurl{doi:#1}}%
}
\DeclareFieldFormat{isbn}{%
  \scriptsize%
  \ifhyperref{%
    \href{https://www.amazon.com/s/?field-keywords=#1}{\nolinkurl{isbn:#1}}%
  }{\nolinkurl{isbn:#1}}%
}

% hide urldate field
\AtEveryBibitem{\clearfield{urlyear}}

% remove period at end of entries
\renewcommand*{\finentrypunct}{}


==> tex/preamble/settings/captions.tex <==
% ======================================================================
% Float Captions
% ======================================================================

% change font size for captions, add horizontal rule
\DeclareCaptionFormat{mycaptionformat}{%
  \small\@hangfrom{#1#2}%
  \advance\caption@parindent\hangindent
  \advance\caption@hangindent\hangindent
  \caption@@par#3\par%
}

\newcommand*{\formatcaption}[1]{%
  \sffamily\bfseries\fontsize{9.5}{12}\selectfont%
  \textls*{\textcolor{mittelblau}{\MakeUppercase{#1}}}%
}

\newcommand*{\formatsubcaption}[1]{%
  \sffamily\bfseries\fontsize{8.8}{11}\selectfont%
  \textls*{\textcolor{mittelblau}{\MakeUppercase{#1}}}%
}

% change appearance of caption label
\DeclareCaptionLabelFormat{mycaptionlabelformat}{%
  \formatcaption{#1 #2}%
}

% special format for unnumbered figures (e.g., cover figure)
\DeclareCaptionLabelFormat{mycaptionlabelformatunnumbered}{%
  \formatcaption{#1}%
}

% set caption format
\captionsetup{
  % use custom format
  format=mycaptionformat,
  % use custom label format
  labelformat=mycaptionlabelformat,
  % separate number and caption with \quad
  labelsep=quad,
}

% don't indent caption text in SCfigure (figures with side caption)
\DeclareCaptionFormat{mysidecaptionformat}{\small#1#2\\#3\par}
\AtBeginEnvironment{SCfigure}{\captionsetup{format=mysidecaptionformat}}
\AtBeginEnvironment{SCtable}{\captionsetup{format=mysidecaptionformat}}

% use maximum space for SCfigure captions (sidecap's default is that
% the caption can only be as wide as the figure itself)
\renewcommand*{\sidecaptionrelwidth}{50}

% change font size for sub-captions
\DeclareCaptionFormat{mysubcaptionformat}{%
  \fontsize{10}{12}\selectfont\@hangfrom{#1#2}%
  \advance\caption@parindent\hangindent
  \advance\caption@hangindent\hangindent
  \caption@@par#3\par%
}

% change appearance of sub-caption label
\DeclareCaptionLabelFormat{mysubcaptionlabelformat}{%
  \formatsubcaption{#2}%
}

% set sub-caption format
\captionsetup[sub]{
  % use custom format
  format=mysubcaptionformat,
  % use custom label format
  labelformat=mysubcaptionlabelformat,
  % separate number and caption with \quad
  labelsep=quad,
}

% use uppercase letters to reference sub-figures
\renewcommand*{\thesubfigure}{\Alph{subfigure}}


==> tex/preamble/settings/checkMode.tex <==
% ======================================================================
% Check Mode
% ======================================================================

% check mode
\iftoggle{checkMode}{
  % show overfull boxes
  \overfullrule=1mm
  % whitelist is in hyphenationWhitelist.txt:
  % one word per line (all lowercase) with dashes (-) indicating the
  % places where hyphenation is permitted
  \LuaCheckHyphen{whitelist=hyphenationWhitelist.txt}
}{}


==> tex/preamble/settings/colors.tex <==
% ======================================================================
% Colors
% ======================================================================

% define line colors (mix between MATLAB and matplotlib colors)
\definecolor{C0}{rgb}{0.000,0.447,0.741}
\definecolor{C1}{rgb}{0.850,0.325,0.098}
\definecolor{C2}{rgb}{0.749,0.561,0.102}
\definecolor{C3}{rgb}{0.494,0.184,0.556}
\definecolor{C4}{rgb}{0.466,0.674,0.188}
\definecolor{C5}{rgb}{0.301,0.745,0.933}
\definecolor{C6}{rgb}{0.635,0.078,0.184}
\definecolor{C7}{rgb}{0.887,0.465,0.758}
\definecolor{C8}{rgb}{0.496,0.496,0.496}

% define university CD colors
\definecolor{anthrazit}{RGB}{62,68,76}
\definecolor{mittelblau}{RGB}{0,81,158}
\definecolor{hellblau}{RGB}{0,190,255}


==> tex/preamble/settings/crossReferences.tex <==
% ======================================================================
% Cross-References
% ======================================================================

% define abbreviated names for cross-references
\crefname{algorithm}{Alg.}{Algorithms}
\Crefname{algorithm}{Algorithm}{Algorithms}

\crefname{chapter}{Chap.}{Chapters}
\Crefname{chapter}{Chapter}{Chapters}

\crefname{corollary}{Cor.}{Corollaries}
\Crefname{corollary}{Corollary}{Corollaries}

\crefname{definition}{Def.}{Definitions}
\Crefname{definition}{Definition}{Definitions}

\crefname{equation}{Eq.}{Equations}
\Crefname{equation}{Equation}{Equations}

\crefname{figure}{Fig.}{Figures}
\Crefname{figure}{Figure}{Figures}

\crefname{lemma}{Lemma}{Lemmas}
\Crefname{lemma}{Lemma}{Lemmas}

\crefname{line}{line}{lines}
\Crefname{line}{Line}{Lines}

\crefname{proposition}{Prop.}{Propositions}
\Crefname{proposition}{Proposition}{Propositions}

\crefname{section}{Sec.}{Sections}
\Crefname{section}{Section}{Sections}

\crefname{table}{Tab.}{Tables}
\Crefname{table}{Table}{Tables}

\crefname{theorem}{Thm.}{Theorems}
\Crefname{theorem}{Theorem}{Theorems}

% reference theorems with their name appended
\newcommand*{\thmref}[1]{\hyperlink{#1}{\cref*{#1}~(\nameref*{#1})}}
\newcommand*{\Thmref}[1]{\hyperlink{#1}{\Cref*{#1}~(\nameref*{#1})}}


==> tex/preamble/settings/dictums.tex <==
% ======================================================================
% Dictums
% ======================================================================

% don't use sans-serif font for dictums
\addtokomafont{dictum}{\rmfamily}

% shortcut for setting the dictum for a chapter
\newcommand*{\setdictum}[3][0.54\textwidth]{%
  \setchapterpreamble{%
    \cleanchapterquote{#1}{#2}{#3}%
    \chapterheadendvskip%
  }%
}

% fancy quotes (taken from cleanthesis.sty, slightly adapted)
\newcommand*{\hugequote}{%
  \fontsize{75}{80}\selectfont%
  \hspace*{-0.6em}\color[rgb]{0.6,0.6,0.6}%
  \textit{``}%
  \vskip -0.8em%
}

\newcommand*{\cleanchapterquote}[3]{%
  \begin{minipage}{\textwidth}%
    \begin{flushright}
      \begin{minipage}{#1}%
        \begin{flushleft}
          {\hugequote}\textit{#2}
        \end{flushleft}
        \begin{flushright}
          \small--- #3
        \end{flushright}
      \end{minipage}%
    \end{flushright}
  \end{minipage}%
  \bigskip
}


==> tex/preamble/settings/dynamic.tex <==
% ======================================================================
% Dynamic Commands
% ======================================================================

% get name of current label (chapter, section, subsection, ...)
\newcommand*{\currentname}{\@currentlabelname}

% calculate difference between page numbers
\newcommand*{\pagedifference}[2]{%
  \number\numexpr\getpagerefnumber{#2}-\getpagerefnumber{#1}\relax%
}

% custom TODO command with warning
% (all packages that were tried produced problems)
\newcommand*{\todo}[1]{%
  \GenericWarning{}{%
    LaTeX Warning (\thesubsection\space\currentname): TODO "#1"%
  }%
  \textcolor{red}{TODO: #1}%
}

% set up versioning information
\edef\gitCommitHash{12ec6c61}
\edef\gitTag{arxiv-v1}
\edef\gitCommitTimeLong{October 11, 2019 at 9:59am}
\edef\currentTimeLong{October 11, 2019 at 10:30am}
\edef\compileCounter{14030}

% convenience commands for title page and watermarks
\newcommand*{\gitCommitText}[1][]{%
  \texttt{#1\gitCommitHash}%
  \ifx\gitTag\empty\else{} (\texttt{#1\gitTag})\fi%
}

\newcommand*{\compileCounterText}[1][]{%
  \texttt{#1v\compileCounter}%
}

% command for checking if file is in \includeonly or not
\newcommand*{\isincluded}[1]{%
  \@tempswatrue
  \if@partsw
    \@tempswafalse
    \edef\reserved@b{#1}%
    \@for\reserved@a:=\@partlist\do
    {\ifx\reserved@a\reserved@b\@tempswatrue\fi}%
  \fi
  \if@tempswa\expandafter\@firstoftwo\else\expandafter\@secondoftwo\fi
}


==> tex/preamble/settings/flipBook.tex <==
% ======================================================================
% Flip Book
% ======================================================================

% prevent "Label `1' multiply defined" warnings when using
% KOMA-Script's \ifthispageodd together with \includeonly
\newcounter{scbookpg}
\renewcommand*{\is@thispageodd}{%
  \@bsphack
  \begingroup
    %\@tempcnta=\scr@tpo
    %\advance\@tempcnta by\@ne
    \stepcounter{scbookpg}%
    \xdef\scr@tpo{\thescbookpg}%
    \protected@write\@auxout{\let\arabic\relax}{%
      \string\new@tpo@label{\scr@tpo}{\arabic{page}}}%
    \expandafter\ifx\csname tpo@\scr@tpo\endcsname\relax
      \protect\G@refundefinedtrue
      \ClassWarning{\KOMAClassName}{%
        odd/even page label number \scr@tpo\space undefined}%
      \edef\@tempa{\the\value{page}}%
    \else
      \edef\@tempa{\csname tpo@\scr@tpo\endcsname}%
    \fi
    \ifodd\number\@tempa
      \aftergroup\thispagewasoddtrue
    \else
      \aftergroup\thispagewasoddfalse
    \fi
  \endgroup
  \@esphack
}

% count pages
\newcounter{currentpagenumber}
\AddEverypageHook{\stepcounter{currentpagenumber}}

% index of current flip book image
\newcount\flipbookindex

% start flip book on dedication page
% (two pages book cover + two pages title page = four pages);
% if in draft mode, add another two pages for the progress table
\newcounter{flipbookstartpagenumber}
\setcounter{flipbookstartpagenumber}{4}
\iftoggle{draftMode}{\addtocounter{flipbookstartpagenumber}{2}}{}

% set up flip book
\iftoggle{flipBookMode}{
  \AddEverypageHook{%
    \flipbookindex=\numexpr(%
      \thecurrentpagenumber-\theflipbookstartpagenumber%
    )/2\relax%
    \ifnum\number\flipbookindex>0%
      \begin{tikzpicture}[remember picture,overlay,scale=1]
        \ifthispageodd{
          \node[anchor=south east,inner sep=0pt,xshift=-7mm,yshift=7mm]
          at (current page.south east) [above left] {%
            \includegraphics[scale=0.8,trim={7mm 10mm 7mm 10mm},clip]{%
              flipBookSG_\number\flipbookindex%
            }%
          };
        }{
          \node[anchor=south west,inner sep=0pt,xshift=7mm,yshift=7mm]
          at (current page.south west) [above right] {%
            \includegraphics[trim={13mm 5mm 10mm 0mm},clip]{%
              flipBookBSpline_\number\flipbookindex%
            }%
          };
        }
      \end{tikzpicture}%
    \fi%
  }
}{}


==> tex/preamble/settings/floats.tex <==
% ======================================================================
% Floats
% ======================================================================

% define mdframed style for floats
\mdfdefinestyle{floatmdfstyle}{
  innerleftmargin=7pt,
  innerrightmargin=7pt,
  innertopmargin=7pt,
  innerbottommargin=6pt,
  roundcorner=10pt,
  linewidth=1pt,
  linecolor=mittelblau,
  backgroundcolor=mittelblau!10,
  % the documentation of mdframed lies about the default values of
  % splittopskip and splitbottomskip
  splittopskip=15pt,
  splitbottomskip=5pt,
  % replace drop shadow with blur shadow
  shadow=true,
  apptotikzsetting={%
    % alternatively, use
    % \tikzset{mdfshadow/.style={blur shadow={shadow blur steps=5}}}%
    % from the pgf-blur package;
    % disadvantage of that is that this uses semi-transparency,
    % which some printers/printing services cannot handle
    % ==> recreate pgf-blur shadow effect with opaque drop shadows
    \tikzset{
      every shadow/.style={shadow xshift=1mm,shadow yshift=-1mm,opacity=1},
      mdfshadow/.style={
        drop shadow={line width=2.4mm,draw=black!03,fill=black!03},
        drop shadow={line width=2.1mm,draw=black!06,fill=black!06},
        drop shadow={line width=1.8mm,draw=black!09,fill=black!09},
        drop shadow={line width=1.5mm,draw=black!12,fill=black!12},
        drop shadow={line width=1.2mm,draw=black!15,fill=black!15},
        drop shadow={line width=0.9mm,draw=black!18,fill=black!18},
        drop shadow={line width=0.6mm,draw=black!21,fill=black!21},
        drop shadow={line width=0.3mm,draw=black!24,fill=black!24},
        drop shadow={draw=none,fill=black!27},
        drop shadow={draw=none,fill=black!30,
                     shadow xshift=0.85mm,shadow yshift=-0.85mm,},
        drop shadow={draw=none,fill=black!33,
                     shadow xshift=0.70mm,shadow yshift=-0.70mm,},
        drop shadow={draw=none,fill=black!36,
                     shadow xshift=0.35mm,shadow yshift=-0.35mm,},
        drop shadow={draw=none,fill=black!39,
                     shadow xshift=0.40mm,shadow yshift=-0.40mm,},
      }
    }%
  },
}

% make "tp" to default position of figure and table
\def\fps@figure{tp}
\def\fps@table{tp}

% don't mix order of figures and tables
% (by default, LaTeX only keeps the order of floats of the same type,
% e.g., figure1-figure2-table1 in the code might display in the order
% figure1-table1-figure1)
\let\ftype@table\ftype@figure

% wrap floats in mdframed boxes,
% automatically center all float contents,
% change font size in float environments
\apptocmd{\@xfloat}{\begin{mdframed}[style=floatmdfstyle]\centering\small}{}{}
\pretocmd{\end@float}{\end{mdframed}}{}{}

% make internal length of sidecap smaller to account for smaller space
% for floats with side captions
\xpatchcmd{\endSC@float}{\endSC@FLOAT\@tempdima}{%
  \setlength{\@tempdima}{\@tempdima-17pt}\endSC@FLOAT\@tempdima%
}{}{}

% automatically center all subfigure contents
\apptocmd{\subcaption@minipage}{\centering}{}{}

% don't move floats to own page (float page) when they are tall,
% the default value is 0.5, which is a bit small
\renewcommand*{\floatpagefraction}{0.73}

% space between floats and text
\setlength{\textfloatsep}{20pt}


==> tex/preamble/settings/glossary.tex <==
% ======================================================================
% Glossary
% ======================================================================

% \newcommand with variable command names
\newcommand*{\newnamecommand}{\@star@or@long\new@name@command}
\newcommand*{\new@name@command}[1]{\expandafter\new@command\csname #1\endcsname}

\iftoggle{partialCompileMode}{
  % define dummy commands that work as if partialCompileMode was disabled
  \newcommand*{\newnotation}[3]{%
    \expandafter\newcommand\csname notationsymbol\string#1\endcsname{#2}%
    \expandafter\newcommand\csname notationtext\string#1\endcsname{#3}%
  }
  \newcommand*{\newnotationcommand}[6][0]{%
    \newcommand*{#2}[#1]{#3}%
    \makecommandnotation{#2}{#4}{#5}{#6}%
  }
  \newcommand*{\newnotationcommandoptarg}[7][]{%
    \newcommand*{#3}[#2][#1]{#4}%
    \makecommandnotation{#3}{#5}{#6}{#7}%
  }
  \newcommand*{\hidenextnotation}{}
  \newcommand*{\makecommandnotation}[4]{%
    \expandafter\newcommand\csname notationsymbol\string#1\endcsname{#3}%
    \expandafter\newcommand\csname notationtext\string#1\endcsname{#4}%
  }
  \newcommand*{\usenotation}[1]{\ignorespaces}
  \newcommand*{\printnotationsymbol}[1]{%
    \csname notationsymbol\string#1\endcsname%
  }
  \newcommand*{\printnotationtext}[1]{%
    \csname notationtext\string#1\endcsname%
  }
  
  \newcommand*{\newgacronym}[3][]{%
    \if\relax\detokenize{#1}\relax%
      \newnamecommand{#2}{\MakeUppercase{#2}\xspace}%
      \newnamecommand{#2s}{\MakeUppercase{#2}s\xspace}%
      \newnamecommand{#2c}{\MakeUppercase{#2}\xspace}%
      \newnamecommand{#2sc}{\MakeUppercase{#2}s\xspace}%
    \else%
      \newnamecommand{#2}{#1\xspace}%
      \newnamecommand{#2s}{#1s\xspace}%
      \newnamecommand{#2c}{\makefirstuc{#1}\xspace}%
      \newnamecommand{#2sc}{\makefirstuc{#1}s\xspace}%
    \fi%
  }
  \newcommand*{\hidegacronym}[1]{}
}{
  % define new glossary style based on long (uses longtable)
  % in which the column widths are fixed and space before/after the
  % table is removed
  \newglossarystyle{longraggedfixed}{
    % base glossary style
    \setglossarystyle{long}
    
    % custom flag to check if we're in the glossary
    \newif\ifinglossary
    
    \renewenvironment{theglossary}%
    {%
      % remove space before/after glossary
      \setlength{\LTpre}{0pt}%
      \setlength{\LTpost}{0pt}%
      %
      % set custom flag that we are now in the glossary
      \inglossarytrue%
      %
      % set font size
      \small%
      %
      % use single spacing
      \begin{spacing}{1}%
        % table header
        \begin{longtable}{@{}L{0.15\textwidth}@{}L{0.85\textwidth}@{}}%
          \textbf{Symbol}\vspace{2mm}&%
          \textbf{Meaning\hfill{}Page with first occurrence}\vspace{2mm}%
          \endhead%
    }%
    {%
      % table footer
        \end{longtable}%
      \end{spacing}%
      % set custom flag that we are now outside the glossary
      \inglossaryfalse%
    }
  
    % add dotted leaders between entry description and page number
    % (called for every row of the table)
    \renewcommand*{\glossentry}[2]{%
      \glsentryitem{##1}\glstarget{##1}{\glossentryname{##1}}&%
      \glossentrydesc{##1}\leavevmode\kern3pt\leaders\hbox{%
        \hspace{0.2237em}.\hspace{0.2237em}%
      }\hfill\kern0pt%
      ##2%
      \tabularnewline%
    }
  }
  
  % use new glossary style
  \setglossarystyle{longraggedfixed}
  
  % add field to glossary entries that stores whether the entry
  % has been used at least once in the document
  \glsaddstoragekey{myused}{false}{\glsmyused}
  \glsaddstoragekey{myisacronym}{false}{\glsmyisacronym}
  
  % \newnotation{sortKey}{entrySymbol}{entryText}
  % adds notation to the glossary without command,
  % only to be used with \usenotation
  \newcommand*{\newnotation}[3]{%
    \newglossaryentry{#1}{text={},sort={#1},name={#2},description={#3}}%
    \expandafter\newcommand\csname notationsymbol\string#1\endcsname{#2}%
    \expandafter\newcommand\csname notationtext\string#1\endcsname{#3}%
  }
  
  % \newnotationcommand[numberOfArgs]{\commandName}
  %   {commandDefinition}{sortKey}{entrySymbol}{entryText}
  % adds notation to the glossary and creates a command
  \newcommand*{\newnotationcommand}[6][0]{%
    \newcommand*{#2}[#1]{#3}%
    \makecommandnotation{#2}{#4}{#5}{#6}%
  }
  
  % \newnotationcommandoptarg[defaultValue]{numberOfArgs}{\commandName}
  %   {commandDefinition}{sortKey}{entrySymbol}{entryText}
  % is like \newnotationcommand, but with an optional argument for
  % the command to be created
  \newcommand*{\newnotationcommandoptarg}[7][]{%
    \newcommand*{#3}[#2][#1]{#4}%
    \makecommandnotation{#3}{#5}{#6}{#7}%
  }
  
  % custom flag to hide the entry defined by the next \newnotationcommand
  % (or similar) from the glossary
  \newif\ifhidenextnotation
  \newcommand*{\hidenextnotation}{\hidenextnotationtrue}
  
  % \makecommandnotation{\commandName}{sortKey}{entrySymbol}{entryText}
  % adds notation to the glossary and modifies \commandName such that
  % the glossary entry is referenced on every use of \commandName
  % (except if used in the glossary itself)
  \newcommand*{\makecommandnotation}[4]{%
    \newglossaryentry{#2}{text={},sort={#2},name={#3},description={#4}}%
    \expandafter\newcommand\csname notationsymbol\string#1\endcsname{#3}%
    \expandafter\newcommand\csname notationtext\string#1\endcsname{#4}%
    \ifhidenextnotation%
      \hidenextnotationfalse%
      \pretocmd{#1}{\glsfieldgdef{#2}{myused}{true}}{}{}%
    \else%
      % only reference entry if outside glossary
      % (otherwise, the page number of the glossary would be displayed)
      \pretocmd{#1}{\ifinglossary\else\usenotation{#2}\fi}{}{}%
    \fi%
  }
  
  % \usenotation{sortKey}
  % explicitly "uses" the notation given by sortKey without printing anything
  \newcommand*{\usenotation}[1]{%
    \glsfieldgdef{#1}{myused}{true}%
    \glsdisp{#1}{\relax}\ignorespaces%
  }
  
  % \printnotationsymbol{\commandName}
  % \printnotationtext{\commandName}
  % print the symbol and the text of the notation given by \commandName
  % if the symbol was created with \makecommandnotation
  % (i.e., \newnotationcommand or \newnotationcommandoptarg);
  % if it was created with \newnotation, use sortKey as argument
  % for \printnotationsymbol and \printnotationtext
  \newcommand*{\printnotationsymbol}[1]{%
    \csname notationsymbol\string#1\endcsname%
  }
  \newcommand*{\printnotationtext}[1]{%
    \csname notationtext\string#1\endcsname%
  }
  
  % shortcut for \newacronym, automatically generating
  % a corresponding shortcut for \gls
  \newcommand*{\newgacronym}[3][]{%
    \if\relax\detokenize{#1}\relax%
      \newacronym[sort={zzzzzzzz#2},description={\makefirstuc{#3}}]%
      {zzzzzzzz#2}{\MakeUppercase{#2}}{#3}%
    \else%
      \newacronym[sort={zzzzzzzz#2},description={\makefirstuc{#3}}]{zzzzzzzz#2}{#1}{#3}%
    \fi%
    \glsfieldgdef{zzzzzzzz#2}{myisacronym}{true}%
    \newnamecommand{#2}{\glsfieldgdef{zzzzzzzz#2}{myused}{true}\gls{zzzzzzzz#2}\xspace}%
    \newnamecommand{#2s}{\glsfieldgdef{zzzzzzzz#2}{myused}{true}\glspl{zzzzzzzz#2}\xspace}%
    \newnamecommand{#2c}{\glsfieldgdef{zzzzzzzz#2}{myused}{true}\Gls{zzzzzzzz#2}\xspace}%
    \newnamecommand{#2sc}{\glsfieldgdef{zzzzzzzz#2}{myused}{true}\Glspl{zzzzzzzz#2}\xspace}%
  }
  
  % hide specific acronyms (that are only used once) in glossary
  \newignoredglossary{hidden}
  \newcommand*{\hidegacronym}[1]{\glsmoveentry{zzzzzzzz#1}{hidden}}
  
  % spell out acronyms at beginning of chapters
  \newcommand*{\resetacronyms}{%
    \forglsentries{\mysymbolname}{%
      \ifthenelse{\equal{\glsmyisacronym{\mysymbolname}}{true}}{%
        \glsreset{\mysymbolname}%
      }{}%
    }%
  }
  
  \addtokomafont{chapter}{\resetacronyms}
  
  % warn for every symbol that has not been used
  \AtEndDocument{%
    \forglsentries{\mysymbolname}{%
      \ifthenelse{\equal{\glsmyused{\mysymbolname}}{false}}{%
        \GenericWarning{}{%
          LaTeX Warning: Symbol ``\mysymbolname'' defined, but unused%
        }%
      }{}%
    }%
  }
  
  % generate table of symbols and acronyms
  \makeglossaries
}

% add debug info about definitions of glossary entries
\iftoggle{showGlossaryDefinitionsMode}{
  \let\oldnewgsymbol\newgsymbol
  \renewcommand*{\newgsymbol}[3]{%
    \ifx\@onlypreamble\@notprerr%
      \textcolor{C1}{Defining ``#2'' as ``#3''. }%
    \fi%
    \oldnewgsymbol{#1}{#2}{#3}%
  }
}{}


==> tex/preamble/settings/graphics.tex <==
% ======================================================================
% Graphics
% ======================================================================

% location of graphics files
\graphicspath{{gfx/}}

% prefer JPGs over PNGs for smaller file size
\DeclareGraphicsExtensions{.pdf,.jpg,.png}

% TikZ libraries
\usetikzlibrary{
  % arrow types
  arrows.meta,
  % coordinate calculations
  calc,
  % zig-zag lines
  decorations.pathmorphing,
  % curly braces
  decorations.pathreplacing,
  % text along paths
  decorations.text,
  % color gradients
  fadings,
  % shadows
  shadows,
}

% set default line width to same as in Matplotlib plots
% created by helper.figure
\tikzset{every picture/.style={line width=1pt}}

% set default arrow tip
\tikzset{>={Stealth[length=5.5pt,width=5.5pt]}}

% draw circle arc around center (standard in TikZ is
% the specification of the first point on the arc)
% [draw options] (center) (initial angle:final angle:radius)
\def\centerarc[#1](#2)(#3:#4:#5){
  \draw[#1] ($(#2)+({(#5)*cos(#3)},{(#5)*sin(#3)})$) arc (#3:#4:#5);
}

% width of contours around text with \contour
\contourlength{1.5pt}


==> tex/preamble/settings/headerFooter.tex <==
% ======================================================================
% Page Headers and Footers
% ======================================================================

% all-caps sans-serif page header
\setkomafont{pageheadfoot}{%
  \normalfont\normalcolor\sffamily%
  \fontsize{9.5}{12}\selectfont\lsstyle%
}
\setkomafont{pagenumber}{\usekomafont{pageheadfoot}\bfseries}

% move page number to page header
\clearscrheadfoot
\lehead[\pagemark]{\pagemark}
\rehead[]{\headmark}
\lohead[]{\headmark}
\rohead[\pagemark]{\pagemark}
\lefoot[]{}
\rofoot[]{}

% prepend "Chapter X: " in front of the chapter name in page headers
\renewcommand*{\chaptermarkformat}{\chapapp{} \thechapter: }


==> tex/preamble/settings/headings.tex <==
% ======================================================================
% Headings
% ======================================================================

% don't use sans-serif font for headings, use single spacing
\setkomafont{disposition}{\normalcolor\bfseries\setstretch{1}}

% format chapter headings with custom commands (below)
\renewcommand*{\chapterformat}{\thechapter}
\renewcommand*{\chapterlinesformat}[3]{\mychapterlinesformat{#2}{#3}}

% check if chapter with number or without number
\newcommand*{\mychapterlinesformat}[2]{%
  \if\relax\detokenize{#1}\relax%
    \chaptertitlenonumber{#2}%
  \else%
    \begin{minipage}{\textwidth}%
      \centering%
      \chapternumber{#1}\\[1em]%
      \chaptertitle{#2}%
    \end{minipage}%
  \fi%
}

% put chapter number in circle
\newcommand*{\chapternumber}[1]{%
  \scalebox{3.0}{%
    \tikz{
      \fill[
        shading=axis,
        left color=mittelblau,
        right color=hellblau,
        shading angle=135,
        inner sep=0mm,
      ] (0,0) circle (5mm);
      \node[
        white,
        inner sep=0mm,
      ] at (0,0) {%
        \ifthenelse{\equal{#1}{3}}{\hspace*{0.4mm}}{}%
        \ifthenelse{\equal{#1}{5}}{\hspace*{0.5mm}}{}%
        \ifthenelse{\equal{#1}{7}}{\hspace*{-0.2mm}}{}%
        \ifthenelse{\equal{#1}{B}}{\hspace*{0.5mm}}{}%
        \ifthenelse{\equal{#1}{C}}{\hspace*{-0.5mm}}{}%
        \ifthenelse{\equal{#1}{D}}{\hspace*{0.5mm}}{}%
        \ifthenelse{\equal{#1}{E}}{\hspace*{0.2mm}}{}%
        \textbf{#1}%
      };
    }%
  }%
}

% if chapter with number: blue chapter title
\newcommand*{\chaptertitle}[1]{\textcolor{mittelblau}{#1}}
% if chapter without number: black chapter title
\newcommand*{\chaptertitlenonumber}[1]{#1}

% set space before and after chapter heading
\RedeclareSectionCommand[beforeskip=5em,afterskip=5em]{chapter}

% Commands for long chapter/section titles:
% If the title is too long, then the mark in the page header will
% overflow and wrap into the next line, which looks ugly.
% \chaptermark/\sectionmark is supposed to fix that. However, if you just
% call it after \chapter/\section, then it will only affect the marks on
% the following pages, not the one on which the heading is defined.
% Therefore, we have to call \chaptermark/\sectionmark twice and also
% supply the optional parameter (otherwise, there will be errors as LaTeX
% tries to add the marks to the table of contents).
% Use the commands like \longchapter{TOC title}{heading title}{mark title}.
\newcommand*{\longchapter}[3]{%
  \chapter[#1]{#2\chaptermark{#3}}\chaptermark{#3}%
}
\newcommand*{\longsection}[3]{%
  \section[#1]{#2\sectionmark{#3}}\sectionmark{#3}%
}
\newcommand*{\addlongchap}[3]{%
  \addchap[#1]{#2\chaptermark{#3}}%
}

% flag to disable ornaments for the next heading
\newif\ifdisableornamentsfornextheading
\disableornamentsfornextheadingfalse

% flag to break before the next heading, but after the ornament
\newif\ifbreakpagebeforenextheading
\breakpagebeforenextheadingfalse

% command to fill up page by manually inserting section ornament
% (for pages with underfull \vbox warnings)
\newcommand*{\fillsectionornament}{%
  \vspace{0ex plus 1fill}\par%
  \hfill\includegraphics{ornament_1}\hfill\null%
  \vspace{-2.125ex plus 1fill}%
  \global\disableornamentsfornextheadingtrue%
}

% command to fill up page by manually inserting subsection ornament
% (for pages with underfull \vbox warnings)
\newcommand*{\fillsubsectionornament}{%
  \vspace{0ex plus 1fil}\par%
  \hfill\includegraphics{ornament_2}\hfill\null%
  \vspace{-1.8ex plus 1fil}%
  \global\disableornamentsfornextheadingtrue%
}

% dirty hack to automatically output ornaments before every section heading
\RedeclareSectionCommand[
  font={%
    \ifdisableornamentsfornextheading%
      \vspace{1.625ex plus .5ex minus -.1ex}%
      \global\disableornamentsfornextheadingfalse%
    \else%
      \hfill\includegraphics{ornament_1}%
      \hfill\null\\[1.625ex plus .5ex minus -.1ex]%
      \ifbreakpagebeforenextheading%
        \pagebreak%
        \global\breakpagebeforenextheadingfalse%
      \else%
        \pagebreak[0]%
      \fi%
    \fi%
    \Large%
  },
  beforeskip=-1.625ex plus -.5ex minus .1ex,
]{section}

% dirty hack to automatically output ornaments before every subsection heading
\RedeclareSectionCommand[
  font={%
    \ifdisableornamentsfornextheading%
      \vspace{1.3ex plus .5ex minus -.1ex}%
      \global\disableornamentsfornextheadingfalse%
    \else%
      \hfill\includegraphics{ornament_2}%
      \hfill\null\\[1.3ex plus .5ex minus -.1ex]%
      \ifbreakpagebeforenextheading%
        \pagebreak%
        \global\breakpagebeforenextheadingfalse%
      \else%
        \pagebreak[0]%
      \fi%
    \fi%
    \large%
  },
  beforeskip=-1.3ex plus -.5ex minus .1ex,
]{subsection}

% decrease skip before \paragraph and \subparagraph headings
\RedeclareSectionCommand[beforeskip=2ex plus 1ex minus .2px]{paragraph}
\RedeclareSectionCommand[beforeskip=1ex plus 1ex minus .2px]{subparagraph}

% append period to \paragraph headings
\let\paragraphwithoutperiod\paragraph
\newcommand*{\paragraphwithperiodwithstar}[1]{\paragraphwithoutperiod*{#1.}}
\newcommand*{\paragraphwithperiod}[1]{\paragraphwithoutperiod{#1.}}
\renewcommand*{\paragraph}{%
  \@ifstar{\paragraphwithperiodwithstar}{\paragraphwithperiod}%
}

% append period to \subparagraph headings
\let\subparagraphwithoutperiod\subparagraph
\newcommand*{\subparagraphwithperiodwithstar}[1]{\subparagraphwithoutperiod*{#1.}}
\newcommand*{\subparagraphwithperiod}[1]{\subparagraphwithoutperiod{#1.}}
\renewcommand*{\subparagraph}{%
  \@ifstar{\subparagraphwithperiodwithstar}{\subparagraphwithperiod}%
}


==> tex/preamble/settings/hyperref.tex <==
% ======================================================================
% PDF Meta-Data and Links
% ======================================================================

% set up hyperref
\hypersetup{
  % set metadata
  pdftitle={\thetitle},
  pdfauthor={\theauthor},
  pdfcreator={LaTeX, KOMA-Script, hyperref},
  % underline links instead of putting a framed box around them
  pdfborderstyle={/S/U/W 1},
  % set link colors
  citebordercolor=C1,
  filebordercolor=C1,
  linkbordercolor=C1,
  menubordercolor=C1,
  runbordercolor=C1,
  urlbordercolor=C0,
  % prepend bookmarks with section number
  bookmarksnumbered,
  % open bookmark tree on start
  bookmarksopen,
}

% include parentheses of \eqref in hyperlink
\renewcommand*{\eqref}[1]{\hyperref[{#1}]{\textup{\tagform@{\ref*{#1}}}}}


==> tex/preamble/settings/initials.tex <==
% ======================================================================
% Initials
% ======================================================================

% indent right of initial
\setlength{\DefaultNindent}{0.5em}
% use height of upper-case letters for height of initial
\renewcommand*{\LettrineSecondString}{X}
% enlarge initial (grows to the top, aligned on baseline of bottom line)
\renewcommand*{\DefaultLoversize}{0.07}
% make initial bold
\renewcommand*{\LettrineFontHook}{\bfseries}
% don't use small caps for rest of first word, make bold
\renewcommand*{\LettrineTextFont}{\normalfont\bfseries}

% custom command: \initial[options]{0.5em}{L}{etter}
% is like \lettrine[options]{L}{etter}, except that the first line
% is moved to the left by 0.5em
\newcommand*{\initial}[4][]{%
  \lettrine[%
    findent=\dimexpr-#2\relax,%
    nindent=\dimexpr#2+\DefaultNindent\relax,%
    #1%
  ]{#3}{#4}%
}


==> tex/preamble/settings/komaTextArea.tex <==
% ======================================================================
% KOMA-Script and Text Area
% ======================================================================

% options for KOMA-Script
\KOMAoptions{
  % choose font size (PO: should be between 12pt and 14pt)
  fontsize=12pt,
  % suppress "very small head height detected" warning
  DIV=12,
  % don't end section numbers with period despite appendices
  numbers=noendperiod,
  % set linespacing of header and footer to 1.5
  % (otherwise, the header will "jump" back and forth from normal
  % pages and pages with single line spacing, e.g., table of contents)
  onpsinit=\onehalfspacing,
  % use \section for headings of list of figures/tables/algorithms
  listof=leveldown,
}

% set page margins
\geometry{
  bindingoffset=25mm,
  inner=10mm,
  outer=20mm,
  top=20mm,
  bottom=30mm,
  includehead=true,
}


==> tex/preamble/settings/mathematics.tex <==
% ======================================================================
% Mathematics
% ======================================================================

% automatically replace "l" with \ell in math mode
\mathcode`l="8000
\begingroup
\lccode`\~=`\l
\DeclareMathSymbol{\lsb@l}{\mathalpha}{letters}{`l}
\lowercase{\gdef~{\ifnum\the\mathgroup=\m@ne \ell \else \lsb@l \fi}}%
\endgroup

% change QED symbol to filled square
\renewcommand*{\qedsymbol}{\textcolor{mittelblau}{$\blacksquare$}}

% redefine own proof environment (prohibits \qedhere)
\renewenvironment{proof}[1][Proof]{%
  \noindent{\formatcaption{#1}\hspace{1em}}%
}{\qed\par}

% siunitx setup
\sisetup{
  % reduce space between units
  inter-unit-product={\hspace{0.03em}},
  % use fractions for inverse units
  per-mode=fraction,
  % use dot for product between number and power of ten
  exponent-product=\cdot,
}

% add \permille macro
\DeclareSIUnit{\permille}{\text{\textperthousand}}

% add \hms command similar to \ang to describe durations
% (e.g., computation times), use as \hms{1;2;3} ==> 1h 02min 03s
\ExplSyntaxOn
\NewDocumentCommand\hms{o>{\SplitArgument{2}{;}}m}{
  \group_begin:
  \IfNoValueF{#1}{\keys_set:nn{siunitx}{#1}}
  \siunitx_hms_output:nnn #2
  \group_end:
}
\cs_new_protected:Npn \siunitx_hms_output:nnn #1#2#3
{
  \IfNoValueF{#1}{
    \tl_if_blank:nF{#1}{
      \SI{#1}{\hour}
      \IfNoValueF{#2}{~}
    }
  }
  \IfNoValueF{#2}{
    \tl_if_blank:nF{#2}{
      \IfNoValueF{#1}{\tl_if_blank:nF{#1}{\sisetup{minimum-integer-digits=2}}}
      \SI{#2}{\minute}
      \IfNoValueF{#3}{~}
    }
  }
  \IfNoValueF{#3}{
    \tl_if_blank:nF{#3}{
      \IfNoValueF{#1}{\tl_if_blank:nF{#1}{\sisetup{minimum-integer-digits=2}}}
      \IfNoValueF{#2}{\tl_if_blank:nF{#2}{\sisetup{minimum-integer-digits=2}}}
      \SI{#3}{\second}
    }
  }
}
\ExplSyntaxOff


==> tex/preamble/settings/metaData.tex <==
% ======================================================================
% Meta-Data
% ======================================================================

% meta-data variables
\newcommand*{\thetitle}{%
  B-Splines for Sparse Grids:\texorpdfstring{\\}{}
  Algorithms and Application to\texorpdfstring{\\}{}
  Higher-Dimensional Optimization%
}
\newcommand*{\theapproval}{%
  Vom Stuttgarter Zentrum für Simulationswissenschaften (SC SimTech) und\\
  der Fakultät für Informatik, Elektrotechnik und Informationstechnik\\
  der Universität Stuttgart zur Erlangung der Würde eines Doktors\\
  der Naturwissenschaften (Dr.\ rer.\ nat.) genehmigte Abhandlung%
}
\newcommand*{\theauthor}{Julian Valentin}
\newcommand*{\thebirthplace}{Stuttgart}
\newcommand*{\thedefensedate}{2.\,April 2019}
\newcommand*{\thedate}{June 2019}
\newcommand*{\theyear}{2019}
\newcommand*{\theuniversity}{Universität Stuttgart}
\newcommand*{\theinstitute}{Institut für Parallele und Verteilte Systeme}
\newcommand*{\theadvisor}{Prof.\ Dr.\ Dirk Pflüger}
\newcommand*{\theexamineri}{Prof.\ Dr.\ Stephen Roberts}
\newcommand*{\theexaminerii}{Prof.\ Dr.-Ing.\ Martin Radetzki}


==> tex/preamble/settings/minitoc.tex <==
% ======================================================================
% Mini Table of Contents
% ======================================================================

% define mdframed style for floats
\mdfdefinestyle{minitocmdfstyle}{
  innerleftmargin=7pt,
  innerrightmargin=7pt,
  innertopmargin=7pt,
  innerbottommargin=6pt,
  roundcorner=10pt,
  linewidth=1pt,
  linecolor=mittelblau,
  backgroundcolor=mittelblau!10,
  % the documentation of mdframed lies about the default values of
  % splittopskip and splitbottomskip
  %splittopskip=15pt,
  %splitbottomskip=5pt,
  % replace drop shadow with blur shadow
  shadow=true,
  apptotikzsetting={%
    % alternatively, use
    % \tikzset{mdfshadow/.style={blur shadow={shadow blur steps=5}}}%
    % from the pgf-blur package;
    % disadvantage of that is that this uses semi-transparency,
    % which some printers/printing services cannot handle
    % ==> recreate pgf-blur shadow effect with opaque drop shadows
    \tikzset{
      every shadow/.style={shadow xshift=1mm,shadow yshift=-1mm,opacity=1},
      mdfshadow/.style={
        drop shadow={line width=2.4mm,draw=black!03,fill=black!03},
        drop shadow={line width=2.1mm,draw=black!06,fill=black!06},
        drop shadow={line width=1.8mm,draw=black!09,fill=black!09},
        drop shadow={line width=1.5mm,draw=black!12,fill=black!12},
        drop shadow={line width=1.2mm,draw=black!15,fill=black!15},
        drop shadow={line width=0.9mm,draw=black!18,fill=black!18},
        drop shadow={line width=0.6mm,draw=black!21,fill=black!21},
        drop shadow={line width=0.3mm,draw=black!24,fill=black!24},
        drop shadow={draw=none,fill=black!27},
        drop shadow={draw=none,fill=black!30,
          shadow xshift=0.85mm,shadow yshift=-0.85mm,},
        drop shadow={draw=none,fill=black!33,
          shadow xshift=0.70mm,shadow yshift=-0.70mm,},
        drop shadow={draw=none,fill=black!36,
          shadow xshift=0.35mm,shadow yshift=-0.35mm,},
        drop shadow={draw=none,fill=black!39,
          shadow xshift=0.40mm,shadow yshift=-0.40mm,},
      }
    }%
  },
}


%\newlength\intextseptemp
%\begingroup
%\setlength\intextseptemp{\intextsep}
%\setlength{\intextsep}{0pt}
\newcommand*{\minitocpagenumberbox}[1]{\small{} (p. #1)}

\newcommand*{\minitoc}[3][0mm]{%
  \begin{wrapfigure}[#3]{r}[15mm]{#2}
    \vspace{-10.5mm}\vspace{#1}%
    \begin{mdframed}[style=minitocmdfstyle]
      {\formatcaption{In this section}}\vspace{0.3em}%
      \small%
      \etocsettocstyle{}{}%
      \etocsetnexttocdepth{subsection}%
      \RedeclareSectionCommands[
        tocraggedpagenumber,
        tocraggedentrytext,
        toclinefill={},
        tocentryindent=0em,
        tocpagenumberbox=\minitocpagenumberbox,
      ]{subsection}%
      \linespread{1}\selectfont%
      \localtableofcontents%
    \end{mdframed}
  \end{wrapfigure}
}
%\setlength\intextsep{\intextseptemp}
%\endgroup


==> tex/preamble/settings/tables.tex <==
% ======================================================================
% Tables
% ======================================================================

% fixed-width column types with left, center, and right alignment
\newcolumntype{L}[1]{%
  >{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}p{#1}%
}
\newcolumntype{D}[1]{%
  >{\centering\let\newline\\\arraybackslash\hspace{0pt}}p{#1}%
}
\newcolumntype{R}[1]{%
  >{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}p{#1}%
}

% colors of table lines and rows
\newcommand*{\tablelinecolor}{mittelblau}
\newcommand*{\headerrowcolor}{mittelblau!40}
\newcommand*{\headerrowtextcolor}{black}
\newcommand*{\oddrowcolor}{mittelblau!10}
\newcommand*{\evenrowcolor}{mittelblau!20}

% \setnumberoftableheaderrows has to be put before every tabular environment,
% sets the \rownum counter such that the 1st content row has row number 1
\newcommand*{\setnumberoftableheaderrows}[1]{%
  \rowcolors{1}{\oddrowcolor}{\evenrowcolor}%
  \global\rownum=\numexpr-#1\relax%
}

% set text color per row, use it like this: \begin{tabular}{=l+l+l+l} ...
% (a single \color command wouldn't suffice, as tabular cells have
% their own boxes, i.e., the font color is reset after every cell)
\newcommand*{\@rowstyle}{}
\newcommand*{\rowstyle}[1]{\gdef\@rowstyle{#1}\@rowstyle\ignorespaces}
\newcolumntype{=}{>{\gdef\@rowstyle{}}C}
\newcolumntype{+}{>{\@rowstyle}C}

% \headerrow has to be put before every tabular header row,
% sets background and text color
\newcommand*{\headerrow}{%
  \rowcolor{\headerrowcolor}%
  \rowstyle{\color{\headerrowtextcolor}}%
}

% automatically select header or odd/even row color
% for the current tabular row
\newcommand*{\autorowcolor}{%
  \ifnum\rownum<1%
    \headerrowcolor%
  \else%
    \ifodd\rownum\oddrowcolor\else\evenrowcolor\fi%
  \fi%
}

% automatically select header or odd/even row color
% for the previous tabular row
\newcommand*{\prevautorowcolor}{%
  \ifnum\rownum<2%
    \headerrowcolor%
  \else%
    \ifodd\rownum\evenrowcolor\else\oddrowcolor\fi%
  \fi%
}

% set thickness of table rules
\setlength{\heavyrulewidth}{0.10em}
\setlength{\lightrulewidth}{0.06em}

% like \toprule, except that the space below the rule has the color
% given in the argument
\newcommand*{\toprulecustom}[1]{%
  \arrayrulecolor{\tablelinecolor}%
  \specialrule{\heavyrulewidth}{\abovetopsep}{0pt}%
  \arrayrulecolor{#1}%
  \specialrule{\belowrulesep}{0pt}{0pt}%
  \arrayrulecolor{black}%
}

% like \midrule, except that the space above and below the rule has the colors
% given in the arguments
\newcommand*{\midrulecustom}[2]{%
  \arrayrulecolor{#1}%
  \specialrule{\aboverulesep}{0pt}{0pt}%
  \arrayrulecolor{\tablelinecolor}%
  \specialrule{\lightrulewidth}{0pt}{0pt}%
  \arrayrulecolor{#2}%
  \specialrule{\belowrulesep}{0pt}{0pt}%
  \arrayrulecolor{black}%
}

% like \bottomrule, except that the space above the rule has the color
% given in the argument
\newcommand*{\bottomrulecustom}[1]{%
  \arrayrulecolor{#1}%
  \specialrule{\aboverulesep}{0pt}{0pt}%
  \arrayrulecolor{\tablelinecolor}%
  \specialrule{\heavyrulewidth}{\belowbottomsep}{0pt}%
  \arrayrulecolor{black}%
}

% commands like \toprule, \midrule, and \bottomrule,
% but automatically guessing the right background colors
% for the spaces above/below the rules
\newcommand*{\toprulec}{\toprulecustom{\autorowcolor}}
\newcommand*{\midrulec}{%
  \midrulecustom{\prevautorowcolor}{\autorowcolor}%
}
\newcommand*{\bottomrulec}{\bottomrulecustom{\prevautorowcolor}}


==> tex/preamble/settings/text.tex <==
% ======================================================================
% Text Body
% ======================================================================

% increase indentation of paragraphs (default: 1em = \quad)
\setlength{\parindent}{2em}

% prohibit inserting page breaks in footnotes
\interfootnotelinepenalty=10000

% only display underfull \hbox/\vbox warnings if really, really bad;
% in a technical text riddled with long inline formulas and narrow
% sub-captions or side-captions, it's just not possible to avoid all
% badnesses over 1000
\hbadness=9999
\vbadness=9999

% mathdesign's Charter font has some questionable kerning between some
% capital letters such as F, P, and V and a period (the space between those
% is far too small); one solution would be to use the charter package for
% the main text, but that leads a number of other issues (the text size is
% then larger, and doesn't match the math font size anymore...)
\newcommand*{\punctfix}[1]{{\hspace{-0.05em}#1}}

% enumerate and itemize spaces
\setlist{
  % space between left edge of text area and left edge of paragraphs
  leftmargin=\parindent,
  % space between item paragraphs (in addition to \parskip)
  itemsep=0pt,
  % space above and below lists
  topsep=0.5em,
}

% math version of \settowidth, automatically choosing the right style
% (textstyle, displaystyle, ...)
\def\mathsettowidth#1#2{%
  \setbox\@tempboxa\hbox{$\m@th\mathpalette{}{#2}$}%
  #1=\wd\@tempboxa%
  \setbox\@tempboxa\box\voidb@x%
}

% \halfhphantom works like \hphantom, except that it creates a box
% that is only half as wide as that of \hphantom
\newlength{\halfhphantomlength}
\newcommand*{\halfhphantom}[1]{%
  \ifmmode%
    \mathsettowidth{\halfhphantomlength}{#1}%
  \else%
    \settowidth{\halfhphantomlength}{#1}%
  \fi%
  \setlength{\halfhphantomlength}{\halfhphantomlength/2}%
  \hspace{\halfhphantomlength}%
}

% \lefthphantom{abc}{defghij} positions the text "abc" as follows:
% |abc    |
%  defghij
\newcommand*{\lefthphantom}[2]{%
  \ifmmode\mathrlap{#1}\else\rlap{#1}\fi%
  \hphantom{#2}%
}

% \centerhphantom{abc}{defghij} positions the text "abc" as follows:
% |  abc  |
%  defghij
\newcommand*{\centerhphantom}[2]{%
  \halfhphantom{#2}%
  \ifmmode\mathclap{#1}\else\clap{#1}\fi%
  \halfhphantom{#2}%
}

% \righthphantom{abc}{defghij} positions the text "abc" as follows:
% |    abc|
%  defghij
\newcommand*{\righthphantom}[2]{%
  \hphantom{#2}%
  \ifmmode\mathllap{#1}\else\llap{#1}\fi%
}

% use Oxford comma for multiple references in cleveref
% (e.g, \cref{fig1,fig2,fig3} => Fig. 1, 2, and 3)
\newcommand*{\creflastconjunction}{, and\nobreakspace}


==> tex/preamble/settings/theorems.tex <==
% ======================================================================
% Theorems
% ======================================================================

% define mdframed style for theorems
\mdfdefinestyle{thmmdfstyle}{
  innerleftmargin=13pt,
  innerrightmargin=7pt,
  innertopmargin=5pt,
  innerbottommargin=6pt,
  linewidth=1pt,
  linecolor=mittelblau,
  backgroundcolor=mittelblau!10,
  % the documentation of mdframed lies about the default values of
  % splittopskip and splitbottomskip
  splittopskip=19pt,
  splitbottomskip=5pt,
  % thick line on left side
  extra={
    \draw[mittelblau,line width=5pt]
    ($(O)+(2.5pt,0pt)$) -- ($(O|-P)+(2.5pt,0pt)$);
  },
}

% "torn page" effect at bottom of the box before page break
\newcounter{mathseed}
\setcounter{mathseed}{3}
\pgfmathsetseed{\arabic{mathseed}}

\tikzset{
  every picture/.append style={
    execute at begin picture={
      \ifboolexpr{
        bool{mdffirstframe} or bool{mdfmiddleframe} or bool{mdflastframe}
      }{
        \mdf@innertikzcalc
        \coordinate (O) at (\mdf@Ox,\mdf@Oy);
        \coordinate (P) at (\mdf@Px,\mdf@Py);
        \ifboolexpr{bool{mdffirstframe} or bool{mdfmiddleframe}}{
          \clip ($(O)+(-0.5pt,2pt)$)
          \pgfextra{
            \addtocounter{mathseed}{1}
            \pgfmathsetseed{\arabic{mathseed}}
          }
          decorate[
            decoration={my random steps,segment length=2pt,amplitude=2pt}
          ]{-- ($(P|-O)+(0.5pt,2pt)$)}
          -- ($(P)+(0.5pt,0.5pt)$)
          -- ($(O|-P)+(-0.5pt,0.5pt)$)
          -- cycle;
        }{}
        \ifboolexpr{bool{mdflastframe} or bool{mdfmiddleframe}}{
          \clip ($(O)+(-0.5pt,-0.5pt)$)
          -- ($(O|-P)+(-0.5pt,-2pt)$)
          \pgfextra{\pgfmathsetseed{\arabic{mathseed}}}
          decorate[
            decoration={my random steps,segment length=2pt,amplitude=2pt}
          ]{-- ($(P)+(0.5pt,-2pt)$)}
          -- ($(P|-O)+(0.5pt,-0.5pt)$)
          -- cycle;
        }{}
      }{}
    }
  }
}

% for the "torn page" effect,
% derived from the "random steps" decoration, the difference is that
% it only add random pertubations in y-direction, not in x-direction
\pgfdeclaredecoration{my random steps}{start}{
  \state{start}[
    width=+0pt,next state=step,
    persistent precomputation=\pgfdecoratepathhascornerstrue
  ]{}
  \state{step}[
    auto end on length=1.5\pgfdecorationsegmentlength,
    auto corner on length=1.5\pgfdecorationsegmentlength,
    width=+\pgfdecorationsegmentlength
  ]{
    \pgfpathlineto{
      \pgfpointadd{
        \pgfpoint{\pgfdecorationsegmentlength}{0pt}
      }{
        \pgfpoint{0pt}{rand*\pgfdecorationsegmentamplitude}
      }
    }
  }
  \state{final}{}
}

% patch mdframed such that it doesn't violate \flushbottom
% (mdframed produces ragged page bottoms without this)
\xpatchcmd{\mdf@put@frame@i}{\hrule \@height\z@ \@width\hsize\vfill}{}{}{}
\xpatchcmd{\mdf@put@frame@i}{\hrule \@height\z@ \@width\hsize\vfill}{}{}{}
\xpatchcmd{\mdf@put@frame@i}{\hrule \@height\z@ \@width\hsize\vfill}{}{}{}

% ignore "bad break" warnings by mdframed, they don't seem to make sense
% (they claim that the box after the page break would be empty,
% even if it isn't)
\WarningFilter{mdframed}{You got a bad break}

% define theorem styles (format theorem "head" with sans-serif caps)
\declaretheoremstyle[
  headformat={\formatcaption{\NAME{} \NUMBER}\hspace{0.7em}\NOTE\\},
  notefont={\normalfont\normalsize},
  headpunct={},
]{mythmdefstyle}

% same as before, but italic body font
\declaretheoremstyle[
  headformat={\formatcaption{\NAME{} \NUMBER}\hspace{0.7em}\NOTE\\},
  notefont={\normalfont\normalsize},
  headpunct={},
  bodyfont={\itshape},
]{mythmplainstyle}

% same as before, but no note and line break after head
\declaretheoremstyle[
  headformat={\formatcaption{\NAME{} \NUMBER}\hspace{0.7em}},
  notefont={\normalfont\normalsize},
  headpunct={},
  bodyfont={\itshape},
]{mythmshortplainstyle}

% theorem environments
\declaretheorem[
  name={Definition},
  numberwithin=chapter,
  mdframed={style=thmmdfstyle},
  style=mythmdefstyle,
]{definition}
\declaretheorem[
  name={Theorem},
  numberlike=definition,
  mdframed={style=thmmdfstyle},
  style=mythmplainstyle,
]{theorem}
\declaretheorem[
  name={Proposition},
  numberlike=definition,
  mdframed={style=thmmdfstyle},
  style=mythmplainstyle,
]{proposition}
\declaretheorem[
  name={Lemma},
  numberlike=definition,
  mdframed={style=thmmdfstyle},
  style=mythmplainstyle,
]{lemma}
\declaretheorem[
  name={Lemma},
  numberlike=definition,
  mdframed={style=thmmdfstyle},
  style=mythmshortplainstyle,
]{shortlemma}
\declaretheorem[
  name={Corollary},
  numberlike=definition,
  mdframed={style=thmmdfstyle},
  style=mythmplainstyle,
]{corollary}
\declaretheorem[
  name={Corollary},
  numberlike=definition,
  mdframed={style=thmmdfstyle},
  style=mythmshortplainstyle,
]{shortcorollary}


==> tex/preamble/settings/toc.tex <==
% ======================================================================
% Tables of Contents, Figures, Tables, Algorithms, and Theorems
% ======================================================================

% remove indentation for lists of figures and tables
\DeclareTOCStyleEntry[indent=0em]{tocline}{figure}
\DeclareTOCStyleEntry[indent=0em]{tocline}{table}

% declare algorithm float environment, create list of algorithms,
% use same formatting as for figures and tables
\DeclareNewTOC[
  type=algorithm,
  name=Algorithm,
  listname={List of Algorithms},
  float,
  floattype=4,
  floatpos=tp,
  counterwithin=chapter,
  tocentrynumwidth=2.3em,
  tocentryindent=0em,
]{loa}

% create list of theorems,
% use same formatting as for figures, tables, and algorithms
% (thmtools's thm-listof.sty is unfortunately a little buggy,
% as it causes the flip book images to jump; using KOMA-Script for
% all lists is more consistent and less error-prone)
\DeclareNewTOC[
  type=mytheorem,
  name=Theorem,
  listname={List of Theorems},
  tocentrynumwidth=2.3em,
  tocentryindent=0em,
]{lop}

% add code that adds the theorem to the *.lop file to hook
\addtotheorempostheadhook{%
  \addxcontentsline{lop}{mytheorem}{\csname ll@\thmt@envname\endcsname}%
}

% use single spacing in
% tables of contents, figures, tables, algorithms, and theorems
\AfterTOCHead{\begin{spacing}{1}}
\AfterStartingTOC{\end{spacing}}

% exclude subsections from table of contents
\setcounter{tocdepth}{\sectionnumdepth}

% increase space of page numbers
% (default values of 1.55em and 2.55em are too small for three-digit numbers)
\renewcommand*{\@pnumwidth}{2em}
\renewcommand*{\@tocrmarg}{3em}


==> tex/preamble/settings/watermarks.tex <==
% ======================================================================
% Watermarks
% ======================================================================

% set up watermarks
\iftoggle{draftMode}{
  \AddEverypageHook{%
    \ifnum\number\thecurrentpagenumber>1%
      \begin{tikzpicture}[remember picture,overlay,scale=1]
        \node[
          anchor=center,xshift=0mm,yshift=7mm,inner sep=0pt,
        ] at (current page.south) [above] {
          \parbox{180mm}{%
            \begin{center}%
              \onehalfspacing\bfseries\color{gray}%
              Draft \compileCounterText[\normalsize{}]
              (\currentTimeShort)\\%
              Commit \gitCommitText[\normalsize{}]
              (\gitCommitTimeShort)%
            \end{center}%
          }%
        };
        \ifthispageodd{
          \node[
            anchor=north east,xshift=-15mm,yshift=-38.5mm,color=gray,
            inner sep=0pt,text width=4.51mm,align=right,
          ] at (current page.north east) [below left] {%
            \ttfamily\onehalfspacing%
            1\\2\\3\\4\\5\\6\\7\\8\\9\\10\\%
            11\\12\\13\\14\\15\\16\\17\\18\\19\\20\\%
            21\\22\\23\\24\\25\\26\\27\\28\\29\\30\\%
            31\\32\\33\\34\\35\\36\\37\\%
          };
        }{
          \node[
            anchor=north west,xshift=15mm,yshift=-38.5mm,color=gray,
            inner sep=0pt,text width=4.51mm,align=right,
          ] at (current page.north west) [below right] {%
            \ttfamily\onehalfspacing%
            1\\2\\3\\4\\5\\6\\7\\8\\9\\10\\%
            11\\12\\13\\14\\15\\16\\17\\18\\19\\20\\%
            21\\22\\23\\24\\25\\26\\27\\28\\29\\30\\%
            31\\32\\33\\34\\35\\36\\37\\%
          };
        }
      \end{tikzpicture}%
    \fi%
  }
}{}


==> tex/preamble/switches.tex <==
% needed for custom switches
\RequirePackage{etoolbox}

% ======================================================================
% Toggle Settings
% ======================================================================

% draftMode switch:
% show draft watermark, disabling overrides checkMode, debugMode, and
% showGlossaryDefinitionsMode (see below)
\newtoggle{draftMode}
\togglefalse{draftMode}

% checkMode switch:
% show all overfull/underfull boxes, show unknown hyphenations
\newtoggle{checkMode}
\toggletrue{checkMode}

% debugMode switch:
% show all boxes, glues, and kerning info
\newtoggle{debugMode}
\togglefalse{debugMode}

% showGlossaryDefinitionsMode switch:
% print definition of glossary entries in the text body
\newtoggle{showGlossaryDefinitionsMode}
\togglefalse{showGlossaryDefinitionsMode}

% flipBookMode switch:
% add flip book images in corners of page
\newtoggle{flipBookMode}
\toggletrue{flipBookMode}

% partialCompile switches:
% only compile a single chapter to save compilation time
\newtoggle{partialCompileMode}
\togglefalse{partialCompileMode}

% select chapters to compile for partialCompileMode = true
\includeonly{%
  %document/10introduction,
  %document/20sparseGrids,
  %document/30BSplines,
  %document/40algorithms,
  %document/50optimization,
  %document/60topoOpt,
  %document/70muscle,
  %document/80finance,
  %document/90conclusion,
  %document/a10proofs,
  %document/a20testProblems,
  %document/a30topoOptDetails,
}

% ======================================================================
% Toggle Logic
% ======================================================================

% disable checkMode, showGlossaryDefinitionsMode, and debugMode
% if draftMode is disabled
\iftoggle{draftMode}{}{
  \togglefalse{checkMode}
  \togglefalse{debugMode}
  \togglefalse{showGlossaryDefinitionsMode}
}

% compile everything if partialCompileMode is disabled
\makeatletter
\iftoggle{partialCompileMode}{}{
  % disable the \includeonly mechanism
  \@partswfalse
}
\makeatother

